Phylogeny-Inspired Adaptation of Multilingual Models to New Languages

Large pretrained multilingual models, trained on dozens of languages, have delivered promising results due to cross-lingual learning capabilities on variety of language tasks. Further adapting these models to specific languages, especially ones unseen during pre-training, is an important goal towards expanding the coverage of language technologies. In this study, we show how we can use language phylogenetic information to improve cross-lingual transfer leveraging closely related languages in a structured, linguistically-informed manner. We perform adapter-based training on languages from diverse language families (Germanic, Uralic, Tupian, Uto-Aztecan) and evaluate on both syntactic and semantic tasks, obtaining more than 20% relative performance improvements over strong commonly used baselines, especially on languages unseen during pre-training.

==> figures/languagefamilies.tex <==
\begin{tikzpicture}
[
    level 1/.style = {red},
    level 2/.style = {blue},
    level 3/.style = {teal},
    every node/.append style = {draw, anchor = west},
    grow via three points={one child at (0.5,-1) and two children at (0.5,-1) and (0.5,-2)},
    edge from parent path={(\tikzparentnode\tikzparentanchor) |- (\tikzchildnode\tikzchildanchor)}]
 
\node {Germanic}
    child {node {West}
    child {node [text width=5cm] {Afrikaans, German, English, Gothic, Low Saxon, Dutch, Swiss German}}
    edge from parent [left]} 
    child [missing] {}
    child [missing] {}
    child {node {North}
    child {node [text width=5cm] {Danish, Faroese, Icelandic, Norwegian, Swedish}}
    edge from parent node [draw = none, left] {}};
\end{tikzpicture}
